Computing Absolutely Normal Numbers in Nearly Linear Time

A real number $x$ is absolutely normal if, for every base $b\ge 2$, every two equally long strings of digits appear with equal asymptotic frequency in the base-$b$ expansion of $x$. This paper presents an explicit algorithm that generates the binary expansion of an absolutely normal number $x$, with the $n$th bit of $x$ appearing after $n$polylog$(n)$ computation steps. This speed is achieved by simultaneously computing and diagonalizing against a martingale that incorporates Lempel-Ziv parsing algorithms in all bases.

==> handwritten.tex <==
I. I


Footnote added.


• • •


d. 2 Jack, can you have a


look at those references?


• • •


2. We prefer to use the notation, f' b) when it refers to the
translation to base b of function f.

• • •


2. I we have revised all our computations and made all calculations
in sections 2, 3 and 4 s except for the computation of dazes , newly
linear time computable in an online fashion, making sure that for
the proof of Theorem 5. I we can diagonalize against d in nearly
linear time.

• • •


Answer to 2. 2:


to mentioned in line 3 of the proof of Theorem


5. t, ru denotes the floor integer part of the square root. Using
this in the minimitation of d??rn) c) is enough to keep × oaf of all
S-Edu].

• • •


2- 3


We corrected base representation to avoid those ending with
infinitely many zeros.


• • •


2. S IT is a r-algebra when endowed with the r-algebra generated by
Cw =3 x e-251W Ex} for w E-2¥. Assuming d G) =L as in construction
4.1, it holds that, for UE-2¥ ouch that {Cw / we we are disjoint and
¥uCw=Zf ? u Nw) =L. ,

• • •


Using the usual correspondence between


25 and C', D (denoted secy, in our paper) the set } Ew] / WE 2-5*4
is a base of the usual r-algebra on co, I], the Borel sets. The
Caratheodory extension can be then used to extend r to all Bowl
sets. Although this is far from trivial, we refrain to include it in
our pager because it can be found

• • •


in classical books on measure theory.


• • •


2. 52 Explained at the beginning of section 2.

• • •


Explained on Z-G


page 6.


• • •


2. 7 Added on page 7.

Let's not do it.


2. 8

2. 9 Done on page 8. Let's not define polynomial boundedness.

2. 10 Done on page i.

2. 11 We have referred to Observation 2. se and Lemma

2. 2. on page 8.

2. 12 Removed

• • •


2- 13, 2.19


Theorem 4.2 already takes care of this in at the end of page 12.


At the end of section 2 we have modified the base-b LZ-martingale,
making it constant for inputs w with Iwls 2b. Therefore polynomial
bounds on b are


polylogarithmic bounds on Iwl.


• • •


2. I 5 explanation added.

2. 16 explanation added.

2. 17 corrected

2. 18 corrected

2. 19 we ignore this

2. 2' added

• • •


2. l add a footnote in page 1 Borel's original definition was that ×
is normal in base b. if X is simply normal in

all bases b, b? b? --- Our definition here is well known to be
equivalent to Borel's.


• • •


B


The structure of this paper is based on the main result proof.
Building on the base-b normality characterisation in terms of finite
state martingales and the universality of hempel-Ziv martingale, we
need to construct a conservative version of the hempel-Ziv marlin-
gale that does not fluctuate too. much and then establish


• • •


a base change method for such conservative martingales. Finally a
careful efficient combination of all resulting strategies for
different bases is needed.


• • •


1


2. I Let ID be the set of dyadic rationals.

• • •


Let f: Eb * ? IR


be a function. f is nearly linear time computable if there exists
no> I and


f: 2- * ? ID such that exactly


i) J is V nearly linear


time computable.


ii t WE-2*5, j E IN


If Cw) -f (w) l Effie


• • •


(I will probably not include this result). Jemima If d: -2¥ > Eo, -3
is a nearly linear time computable martingale then there exist d':
-2¥ ? ID an exactly nearly linear time computable martingale such
that 5- [d) = S- [d'].


• • •


d' G) = da) Puff


sketch


d' (wa) =


d 'Cw) + Ic wa) (t's)


I Icwb') -Lb b't a be proven

Then it can that:


. d' is a martingale


S- [d'] = S-Ed]

d" is nearly linear time co-portable.

• • •


IR


*

Let f: 2b


be a function. f is nearly linear time computable in an online
fashion if there exists


It g: 2b IR ouch that is f, g are nearly linear time computable. i i
V a E E b s f (wa), g (wa) can be computed in polfog time from

• • •


w, fcw), gcw).


• • •


Lemma For each online nearly linear time computable super martingale
d. there is a nearly linear time computable martingale d' with S-Ed]
E S-L-d']. If d is polinomially bounded (that is , there is a, b> 0
with


d. (w) Eal w lb for every w), then d' is also polinomially bounded.


.


• • •


Proof


we define d' recursively as follows,


d. 'G) =D Ca) d. " (wa) =D (wa) t


+ d' Cw)


I § d Cwb')

The following can be proven by induction


1. d 'Cw)> dew)

2. d' is a martingale

3. d 'Cuse-2 dew) (l-f) C

UEW


• • •


And clearly d" is online nearly linear time computabl and
polinomially bounded if d is so.


• • •


d' C w) E d Cw). c


d' Cw a) E d Cw a) t


d Cw). C


f-2 d C w b')

(l-f) d Cw a)


d Cw)> Idea)


b d' Cw a) E Z d (y). (I-


y E wa H d 'Cwa) Ef-f) dewaltyEwdgkt's)


• • •


o. 6


Before Notice...


Notice that the function


h Cw) = (Tcw), × (w), Lex, w),


Dcw)) is nearby linear time computable in an online fashion.


2. l 2

• • •


Observation 2.2 There is a C such that for all n E Ab,


2. I

3


facto (n) =


C o n" e-Cn-Dk-D. h "2. ecb-1) 42 4h e-C b- 177720¥ e C b-175/30240#
e O C kn 7)


r


• • •


Let


facto (n) =


C o n" e-Cn-Dk-D. h "2. ecb-1) 42 4h e-C b- 137720¥ e C b-175/30240
¥


Notice that we compute faith (n) with an approxi­mation e O' "n",
that is, all terms in the exponents have precision 7- Gut old).


• • •


A


In order to avoid lime bounds that are dependent on the alphabet
size b, we will consider the following variant of ducts) '


b (WIC 2 ¥1 b) (w) = §dLzCb??


? (b) (wi 25 if I 17 2b.


W


, o' . Notice that ?Edy,] -­5- [due by] and-1£ any unbounded f , Sf
[du. as] = SSE#Eb)].


• • •


Notice that if eglwl> b then a polynomial bound. on b
isopolylogaritmical bound on 1W!.


• • •


p. 10


Proof of claim 3.9


2. I we first proof that e': -3*-3 IR can be computed in nearly
linear time in an online fashion. Let

1W ????. Lcw). b- taken G) I'Cw) = b


fact, 4


• • •


I e' Cw) -en' (w) l E


b, wi-taken (w) ((w).


facts Dew D- ¥CDcwT) ? btw I-taken Cw)

L (w) . facts (Dew))-facts (DW) facts (Dew)). fatty Deus) bi
wi-taken Cw)L (w)

E


(l-elbow??


facts (Dew)) = e' (w). (I-Elbow")


• • •


I e' Cw) -en' (w) l E


e' Cw) ???t÷; t--J


I e' Cw) -en' Cw) / E


e' Cw) -z' ??+ to (Dfw, Eb Dfw). LC a) ftp.#.tolbTwsH


E b I iz notice that CDcwj5 + 0 (&)


D. (w) z TE, therefore I e' Cw) -en 'Cust e be??s t ?


• • •


I' b computable


linear time in Since


in nearly


an online fashion, e' is too.


• • •
------------------------

Since dcwdedcwci.es) it holds that E' " ' 'zu-29dam-outs) b- I


? E' " 'II-FIucwc)=dCwe)


u=, g41wHzIuI§u(word) EdCwCieD=Z


U=1 ? 8¥''- 'Z-u-EYducwu-cdtc.IT


4=1


5


• • •


Therefore


? wt ti) z-u-2??du (wa) z


U = I


? ¥4't'}-u-2rad. (wei-d) t


u = I


+ ?? ' " 'EY,÷,


he = 1


Since du 's a martingale, Eau't'} -u-Eduard E Z


"='gzawHDg-u-2Fdu (w) t


2 "=' gym, ti) z-U-2K2g 1- ¥ I quit 133 U = I

• • •


And


d Cwc) ? ??w't'} -u-zoa


(ducwdtwt.is U=1 ? ??w't} -u-2% (w)


U =L


y?witDzu-Fez


Z - U = I feel + g) 3 ? Ew' 2" -FIU Cw) t


U = I


? t')z_u-F?? Z


h = I


epawlti) z-u-Fdu (w) t I


U=f4wIt I


? + 2- (tutti


• • •


? dew)t-22" -2%3­6=1 (WITI


+ #wit D 2- u-Itzlwl


2


h=g2CcwDt1


E d Cw) t Yawp .


)3


• • •


we agitate


& a. art""??


or oyeeify einem


r vie Let d' be tdmartingale with S-L-d] E S- [d'] constructed in
lemma 2. x. Notice that since


d' Cw)> dew) 6


g' is a savings account for d'.


==> resto1.tex <==

In this paper we present a new algorithm that provably computes an
absolutely normal in nearly linear time.  Our algorithm computes the
binary expansion of an absolutely normal number $x$, with the $n$th
bit of $x$ appearing after $O(n\polylog(n))$ steps. The term
``nearly linear time'' was introduced by Gurevich and Shelah
\cite{GurShe89}. In that paper they showed that, while linear time
computability is very model-dependent, nearly linear time is very
robust.  For example, they showed that random access machines,
Kolmogorov-Uspensky machines, Schoenhage machines, and random-access
Turing machines share exactly the same notion of nearly linear time.

Our algorithm uses the Lempel-Ziv parsing algorithm to achieve its
nearly linear time bound.  For each base $b\ge 2$, we use a
martingale (betting strategy) that employs the Lempel-Ziv parsing
algorithm and is implicit in the work of Feder \cite{Fede91}. This
base-$b$ Lempel-Ziv martingale succeeds exponentially when betting
on the successive digits of the base-$b$ expansion of any real
number that is not normal in base $b$.  Our algorithm simultaneously
computes and diagonalizes against (limits the winnings of) a
martingale that incorporates efficient proxies of all these
martingales, thereby efficiently computing a real number that is
normal in every base.

The rest of this paper is organized as follows.  Section \ref{sec2}\
presents the base-$b$ Lempel-Ziv martingales and their main
properties.  Section \ref{sec3}\  shows how to transform a base-$b$
Lempel-Ziv martingale into a base-$b$ martingale with an efficiently
computable nondecreasing savings account that is unbounded whenever
the base-$b$ Lempel-Ziv martingale succeeds exponentially. Section
\ref{sec4}\ develops an efficient method for converting a base-$b$
martingale with an efficiently computable savings account to a
base-2 martingale that succeeds whenever the base $b$ savings
account is unbounded. Section \ref{sec5}\ presents an algorithm that
exploits the uniformity of these constructions to efficiently and
simultaneously compute (a) a single base-2 martingale $d$ that
succeeds on the binary expansion of every real number $x$ for which
some base-$b$ martingale succeeds on the base-$b$ expansion of $x$
and (b) a particular real number $x$ on which binary expansion $d$
does not succeed. This $x$ is, perforce, absolutely normal. Section
\ref{sec6}\ presents an open problem related to our work.

